Lagrangian Zigzag Cobordisms

We investigate an equivalence relation on Legendrian knots in the standard contact three-space defined by the existence of an interpolating zigzag of Lagrangian cobordisms. We compare this relation, restricted to genus-$0$ surfaces, to smooth concordance and Lagrangian concordance. We then study the metric monoid formed by the set of Lagrangian zigzag concordance classes, which parallels the metric group formed by the set of smooth concordance classes, proving structural results on torsion and satellite operators. Finally, we discuss the relation of Lagrangian zigzag cobordism to non-classical invariants of Legendrian knots.

==> macros.tex <==
\pdfminorversion=7

\makeatletter
\g@addto@macro\@floatboxreset\centering
\makeatother

\def\mathcenter#1{%
  \vcenter{\hbox{$#1$}}%
}

\allowdisplaybreaks[4]

\addto\extrasamerican{%
  \def\sectionautorefname{Section}%
  \def\subsectionautorefname{Section}%
  \def\subsubsectionautorefname{Section}%
}

\let\fullref\autoref

\newtheorem{theorem}{Theorem}[section]
\newtheorem{maintheorem}{Theorem}[section]
\newtheorem{corollary}{Corollary}[section]
\newtheorem{maincorollary}{Corollary}[section]
\newtheorem{proposition}{Proposition}[section]
\newtheorem{lemma}{Lemma}[section]

\theoremstyle{definition}
\newtheorem{definition}{Definition}[section]
\newtheorem{remark}{Remark}[section]
\newtheorem{example}{Example}[section]
\newtheorem{question}{Question}[section]
\newtheorem{openquestion}{Open Question}[section]

\makeatletter
\let\c@maintheorem=\c@theorem
\let\c@corollary=\c@theorem
\let\c@maincorollary=\c@theorem
\let\c@proposition=\c@theorem
\let\c@lemma=\c@theorem
\let\c@remark=\c@theorem
\let\c@example=\c@theorem
\let\c@question\c@theorem
\let\c@definition=\c@theorem
\let\c@equation\c@theorem
\let\c@openquestion\c@theorem
\makeatother

\def\makeautorefname#1#2{\expandafter\def\csname#1autorefname\endcsname{#2}}

\makeautorefname{maintheorem}{Theorem}%
\makeautorefname{maincorollary}{Corollary}%
\makeautorefname{theorem}{Theorem}%
\makeautorefname{corollary}{Corollary}%
\makeautorefname{proposition}{Proposition}%
\makeautorefname{lemma}{Lemma}%
\makeautorefname{example}{Example}%
\makeautorefname{remark}{Remark}%
\makeautorefname{definition}{Definition}%
\makeautorefname{question}{Question}%

\numberwithin{equation}{section}

%\let\origtheequation\theequation
%\makeatletter
%\def\tagform@#1{\maketag@@@{\ignorespaces#1\unskip\@@italiccorr}}
%\makeatother
%\renewcommand{\theequation}{(\origtheequation)}
%
%\renewcommand{\thesubfigure}{\textsc{\alph{subfigure}}}
%
%\newcommand*{\Alphabet}{ABCDEFGHIJKLMNOPQRSTUVWXYZ1234567890}
%\newcommand*{\alphabet}{abcdefghijklmnopqrstuvwxyz1234567890}
%\newlength\Lcaph
%\newlength\Ldesc
%\newlength\Lactualfontsize
%\settoheight{\Lcaph}{\Large \Alphabet}
%\settodepth{\Ldesc}{\Large \Alphabet \alphabet}
%\setlength{\Lactualfontsize}{\dimexpr\Lcaph+\Ldesc\relax}
%\newlength\scaph
%\newlength\sdesc
%\newlength\sactualfontsize
%\settoheight{\scaph}{\small \Alphabet}
%\settodepth{\sdesc}{\small \Alphabet \alphabet}
%\setlength{\sactualfontsize}{\dimexpr\scaph+\sdesc\relax}
%\newlength\scrcaph
%\newlength\scrdesc
%\newlength\scractualfontsize
%\settoheight{\scrcaph}{\small \Alphabet}
%\settodepth{\scrdesc}{\small \Alphabet \alphabet}
%\setlength{\scractualfontsize}{\dimexpr\scrcaph+\scrdesc\relax}
%
%\let\itensor\tensor
%
%\setlength{\multicolsep}{2.27498pt plus 2.27498pt}


